Adapting Surprise Minimizing Reinforcement Learning Techniques for Transactive Control

Optimizing prices for energy demand response requires a flexible controller with ability to navigate complex environments. We propose a reinforcement learning controller with surprise minimizing modifications in its architecture. We suggest that surprise minimization can be used to improve learning speed, taking advantage of predictability in peoples' energy usage. Our architecture performs well in a simulation of energy demand response. We propose this modification to improve functionality and save in a large scale experiment.

==> sections/fixedload-results.tex <==
\subsection{Fixed load sampling}
\subsubsection{Problem Statement}
We suppose that sometimes learning can happen in unrealistic and undesirable ways. 
Consider a controller that simply raises the prices arbitrarily, or reduces prices arbitrarily. 
We propose that the samples of prices should be with respect to a constant load of magnitude $ c$. 
This way the price vector across the the day is equal to 
\begin{align*}
  P &= c p_1 + c p_2 + \ldots c p_{10} \\
    &= c(p_1 + p_2 + \ldots p_{10}) \\
    &= c \lVert \vec{p} \rVert_1
\end{align*}
So the magnitude is constant. 
\subsubsection{L1 Norm}
We observe that now our problem is equivalent to sampling $ \vec{p}$ with a fixed L1 norm. 

\includegraphics[width=2cm]{graphics/box_uniform.png} $\rightarrow$  \includegraphics[width=2cm]{graphics/tri_uniform.png}
    
    
\red{Will idk what you want to add here. Sorry for the late addition.}

